Spatial distribution of small hydrocarbons in the neighborhood of the Ultra Compact HII region Monoceros R2

We study the chemistry of small hydrocarbons in the photon-dominated regions (PDRs) associated with the ultra-compact HII region Mon R2. Our goal is to determine the variations of the abundance of small hydrocarbons in a high-UV irradiated PDR and investigate their chemistry. We present an observational study of CH, CCH and c-C$_3$H$_2$ in Mon R2 combining data obtained with the IRAM 30m telescope and Herschel. We determine the column densities of these species, and compare their spatial distributions with that of polycyclic aromatic hydrocarbon (PAH). We compare the observational results with different chemical models to explore the relative importance of gas-phase, grain-surface and time-dependent chemistry in these environments. The emission of the small hydrocarbons show different patterns. The CCH emission is extended while CH and c-C$_3$H$_2$ are concentrated towards the more illuminated layers of the PDR. The ratio of the column densities of c-C$_3$H$_2$ and CCH shows spatial variations up to a factor of a few, increasing from $N(c-C$_3$H$_2$)/N(CCH)\approx0.004$ in the envelope to a maximum of $\sim0.015-0.029$ towards the 8$\mu$m emission peak. Comparing these results with other galactic PDRs, we find that the abundance of CCH is quite constant over a wide range of G$_0$, whereas the abundance of c-C$_3$H$_2$ is higher in low-UV PDRs. In Mon R2, the gas-phase steady-state chemistry can account relatively well for the abundances of CH and CCH in the most exposed layers of the PDR, but falls short by a factor of 10 to reproduce c-C$_3$H$_2$. In the molecular envelope, time-dependent effects and grain surface chemistry play a dominant role in determining the hydrocarbons abundances. Our study shows that CCH and c-C$_3$H$_2$ present a complex chemistry in which UV photons, grain-surface chemistry and time dependent effects contribute to determine their abundances.

==> authors.tex <==
\author{
P.~Pilleri\inst{1,2,3},
S.~Trevi\~no-Morales\inst{4},
A.~Fuente\inst{2}, 
C.~Joblin\inst{5,6},
J.~Cernicharo\inst{1},
M.~Gerin\inst{7},
S.~Viti\inst{8},
O.~Bern\'e\inst{5,6},
J.R.~Goicoechea\inst{1},
J.~Pety\inst{9},
M.~Gonzalez-Garc\'ia\inst{4},
J.~Montillaud\inst{10},
V.~Ossenkopf\inst{11},
C.~Kramer\inst{4},
S.~Garc{\'i}a-Burillo\inst{2},
F.~Le~Petit\inst{12},
J.~Le~Bourlot\inst{12}
}


 \institute{%
 %1
Centro de Astrobiolog\'{\i}a (INTA-CSIC),
             Ctra. M-108, km.~4, E-28850 Torrej\'on de Ardoz, Spain
\and
%2
Observatorio Astron\'omico Nacional, Apdo. 112, E-28803 Alcal\'a de Henares (Madrid), Spain
\and
Los Alamos National Laboratory, Los Alamos, NM 87545, USA
\and
%3
Instituto de Radio Astronom\'ia Milim\'etrica (IRAM), Avenida Divina Pastora 7, Local 20, 18012 Granada, Spain
%4
\and
Universit\'e de Toulouse; UPS-OMP; IRAP;  Toulouse, France
\and
%5
CNRS; IRAP; 9 Av. colonel Roche, BP 44346, F-31028 Toulouse cedex 4, France 
\and
LERMA, Observatoire de Paris, 61 Av. de l'Observatoire, 75014 Paris, France 
\and
%6
Dept. of Physics and Astronomy, UCL, Gower Place, London WC1E6BT, UK
\and
%7
Institut de Radioastronomie Millim\'etrique, 300 Rue de la Piscine, 38406 Saint Martin d'H\'eres, France
 \and
 %8
Department of Physics, P.O.Box 64, FI-00014, University of Helsinki, Finland
\and
%10
 I. Physikalisches Institut der Universit\"at zu K\"oln, Z\"ulpicher Stra\ss{}e 77, 50937 K\"oln, Germany
\and
%9
Observatoire de Paris, LUTH and Universit\'e Denis Diderot, Place J.
Janssen, 92190 Meudon, France
}
%
%\and
%4
% SRON Netherlands Institute for Space Research, P.O. Box 800, 9700 AV 
% Groningen, Netherlands
% \and
%5
% Leiden Observatory, Universiteit Leiden, P.O. Box 9513, NL-2300 RA Leiden, The Netherlands  \and
% %6
%
%\and
%7
%
% \and
% %8
%%10
%%\and
%%11
%Observatoire de Paris, LUTH and Universit\'e Denis Diderot, Place J.
%Janssen, 92190 Meudon, France
%



% \author{A.~Fuente\inst{1}, O.~Bern\'e\inst{2}, J.~Cernicharo\inst{3},
% J.R.~Rizzo\inst{3}, M.~Gonz\'alez-Garc\'{\i}a\inst{4}, J.R.~Goicoechea\inst{3}
% P.~Pilleri\inst{5,6}, V.~Ossenkopf\inst{7,8}, M. Gerin\inst{9}, R.~G\"usten\inst{10},
% M.~Akyilmaz\inst{7}, A.O.~Benz\inst{11}, F.~Boulanger\inst{12}, S.~Bruderer\inst{11},
% C.~Dedes\inst{11}, K.~France\inst{13}, S. Garc\'{\i}a-Burillo\inst{14}, A.~Harris\inst{15},
% C.~Joblin\inst{5,6}, T.~Klein\inst{10}, C.~Kramer\inst{4}, F.~Le Petit\inst{16}, 
% S.D.~Lord\inst{17}, P.G.~Martin\inst{13}, J.~Mart\'{\i}n-Pintado\inst{3},B.~Mookerjea\inst{18},
% D.A.~Neufeld\inst{19}, Y.~Okada\inst{7}, J. Pety\inst{20}, T.G.~Phillips\inst{21}, M.~R\"ollig\inst{7},
% R.~Simon\inst{7}, J.~Stutzki\inst{7}, F.~van der Tak\inst{8,22},D.~Teyssier\inst{23}, A. Usero\inst{14},
% H.~Yorke\inst{24}, K.~Schuster\inst{20}, M. Melchior\inst{25}, A.~Lorenzani\inst{26}, R. Szczerba\inst{27},
% M.~Fich\inst{28}, C.~McCoey\inst{28,29}, J. Pearson\inst{24}, P.~Dieleman\inst{30}}
% 
% \institute{
% Observatorio Astron\'omico Nacional (OAN), Apdo. 112, 28803 Alcal\'a de Henares (Madrid), Spain
% \and
% Leiden Observatory, Universiteit Leiden, P.O. Box 9513, NL-2300 RA Leiden, The Netherlands 
% \and
% Centro de Astrobiolog\'ia, CSIC-INTA, 28850, Madrid, Spain
% \and
% Instituto de Radio Astronom\'ia Milim\'etrica (IRAM), Avenida Divina Pastora 7, Local 20, 18012 Granada, Spain
% \and
% Universit\'e de Toulouse, UPS, CESR, 9 avenue du colonel Roche, 31062 Toulouse cedex 4, France
% \and
% CNRS, UMR 5187, 31028 Toulouse, France
% \and
% I. Physikalisches Institut der Universit\"at 
% zu K\"oln, Z\"ulpicher Stra\ss{}e 77, 50937 K\"oln, Germany
% \and
% SRON Netherlands Institute for Space Research, P.O. Box 800, 9700 AV 
% Groningen, Netherlands
% \and
% LERMA, Observatoire de Paris, 61 Av. de l'Observatoire, 75014 Paris, France 
% \and
% Max-Planck-Institut f\"ur Radioastronomie, Auf dem H\"ugel 69, 53121, Bonn, Germany
% \and
% Institute for Astronomy, ETH Z\"urich, 8093 Z\"urich, Switzerland
% \and
% Institut d'Astrophysique Spatiale, Universit\'e Paris-Sud, B\^at. 121, 91405 Orsay Cedex, France
% \and
% Department of Astronomy and Astrophysics, University of Toronto, 60 St. George Street, Toronto, ON M5S 3H8, Canada
% \and
% Observatorio Astron\'omico Nacional (OAN), Alfonso XII, 3, 28014 Madrid, Spain
% \and
% Astronomy Department, University of Maryland, College Park, MD 20742, USA
% \and
% Observatoire de Paris, LUTH and Universit\'e Denis Diderot, Place J. Janssen, 92190 Meudon, France
% \and
% IPAC/Caltech, MS 100-22, Pasadena, CA 91125, USA
% \and 
% Tata Institute of Fundamental Research (TIFR), Homi Bhabha Road, Mumbai 400005, India
% \and 
% Department of Physics and Astronomy, Johns Hopkins University, 3400 North Charles Street, Baltimore, MD 21218, USA
% \and
% Institut de Radioastronomie Millim\'etrique, 300 Rue de la Piscine, 38406 Saint Martin d'H\'eres, France
% \and
% California Institute of Technology, 320-47, Pasadena, CA  91125-4700, USA
% \and
% Kapteyn Astronomical Institute, University of Groningen, PO box 800, 9700 AV Groningen, Netherlands
% \and
% European Space Astronomy Centre, Urb. Villafranca del Castillo, P.O. Box 50727, Madrid 28080, Spain
% \and
% Jet Propulsion Laboratory, 4800 Oak Grove Drive, Pasadena, CA 91109  U.S.A.
% \and
% Institut für 4D-Technologien, FHNW, 5210 Windisch, Switzerland 
% \and
% Osservatorio Astrofisico di Arcetri-INAF- Largo E. Fermi 5 I-50100 Florence, Italy 
% \and
% N. Copernicus Astronomical Center, Rabianska 8, 87-100, Torun, Poland 
% \and
% Department of Physics and Astronomy, University of Waterloo, Waterloo, ON Canada N2L 3G1 
% \and
% University of Western Ontario, Dept. of Physics \& Astronomy, London,
% Ontario, Canada N6A 3K7
% \and
% SRON Netherlands Institute for Space Research, Landleven 12, 9747 AD Groningen
% }

